Superpolynomial Lower Bounds for Decision Tree Learning and Testing

We establish new hardness results for decision tree optimization problems, adding to a line of work that dates back to Hyafil and Rivest in 1976. We prove, under randomized ETH, superpolynomial lower bounds for two basic problems: given an explicit representation of a function $f$ and a generator for a distribution $\mathcal{D}$, construct a small decision tree approximator for $f$ under $\mathcal{D}$, and decide if there is a small decision tree approximator for $f$ under $\mathcal{D}$. Our results imply new lower bounds for distribution-free PAC learning and testing of decision trees, settings in which the algorithm only has restricted access to $f$ and $\mathcal{D}$. Specifically, we show: $n$-variable size-$s$ decision trees cannot be properly PAC learned in time $n^{\tilde{O}(\log\log s)}$, and depth-$d$ decision trees cannot be tested in time $\exp(d^{\,O(1)})$. For learning, the previous best lower bound only ruled out $\text{poly}(n)$-time algorithms (Alekhnovich, Braverman, Feldman, Klivans, and Pitassi, 2009). For testing, recent work gives similar though incomparable bounds in the setting where $f$ is random and $\mathcal{D}$ is nonexplicit (Blais, Ferreira Pinto Jr., and Harms, 2021). Assuming a plausible conjecture on the hardness of Set-Cover, we show our lower bound for learning decision trees can be improved to $n^{\Omega(\log s)}$, matching the best known upper bound of $n^{O(\log s)}$ due to Ehrenfeucht and Haussler (1989). We obtain our results within a unified framework that leverages recent progress in two lines of work: the inapproximability of Set-Cover and XOR lemmas for query complexity. Our framework is versatile and yields results for related concept classes such as juntas and DNF formulas.

==> main_hardness.tex <==


\section{Hardness of learning} 
\label{sec:hardness} 

\lnote{I made a pass over the stuff that's grayed-out below and rewrote it in~\Cref{sec:DT-construction}.} 

\gray{ \subsection{Key structural result: from gapped {\sc Set Cover} to gapped decision trees} 

Given a set cover instance $\mathcal{S}=(S,U,E)$ we construct a function $\Gamma_{\mathcal{S}}:\zo^{|S|}\to\zo$ and a distribution $\mathcal{D}_\mathcal{S}$ whose $k$-junta/decision tree complexity closely relates to the set cover complexity of $\mathcal{S}$. 
% \begin{definition}[$\mathcal{D}_S$ and $\Gamma_S$]
% \label{def:f_S}
% Let $\mathcal{S}=(S,U,E)$ be a set cover instance with $|S|=n$. Then $\mathcal{D}_\mathcal{S}$ is the distribution over $\zo^{n}$ given by $\Pr[x=0^n]=1/2$, and for all $u\in U$, $\Pr[x=u]=1/(2|U|)$ where a vertex $u\in U$ is identified by its neighborhood set $\mathcal{N}_\mathcal{S}(u)$ viewed as an indicator vector in $\zo^n$. Then define the function $\Gamma_\mathcal{S}:\supp(D)\to\zo$ by 
% $$
% \Gamma_\mathcal{S}(x)=
% \begin{cases}
% 0 & x=0^n\\
% 1 & x=u, u\in U.
% \end{cases}
% $$
% \end{definition}

\begin{definition}[$\mathcal{D}_S$ and $\Gamma_S$]
%\label{def:D_S_and_Gamma_S}
Let $\mathcal{S}=(S,U,E)$ be a set cover instance with $|S|=n$. Then $\mathcal{D}_\mathcal{S}$ is the distribution over $\zo^{n}$ given by $\Pr[x=1^n]=1/2$, and for all $u\in U$, $\Pr[x=u]=1/(2|U|)$ where a vertex $u\in U$ is identified by the complement of its neighborhood set $S\setminus \mathcal{N}_\mathcal{S}(u)$ viewed as an indicator vector in $\zo^n$.\footnote{We take the complement since the ``top'' string is $1^n$. This order is necessary to later obtain hardness against DNFs. If instead, one were interested in proving hardness against CNFs, then one would take the string $0^n$ as the ``bottom'' string and the strings $N_\mathcal{S}(u)$ directly.}\lnote{Identifying a vertex with the indicator of the complement of its neighborhood is quite confusing (and I don't think most readers will understand what we're saying in the footnote). I think we should switch back to disjunctions instead of conjunctions} Then define the function $\Gamma_\mathcal{S}:\supp(D)\to\zo$ by 
$$
\Gamma_\mathcal{S}(x)=
\begin{cases}
1 & x=1^n\\
0 & x=u, u\in U.
\end{cases}
$$
\end{definition}

When $\mathcal{S}$ is clear from context we will drop the subscript and simply write $\Gamma$ and $\mathcal{D}$. The set cover instance is ``encoded'' in the distribution $\mathcal{D}$ and the function $\Gamma$ in the sense that determining the relevant variables of the function is equivalent to computing a set cover. Indeed, any size-$k$ set cover corresponds to a monotone conjunction that computes $\Gamma$ exactly over\lnote{Consistency check: are we going with ``under" or ``over" a distribution?  I use the former in the introduction, but happy to switch.} the distribution $D$.

\begin{fact}
%\label{fact:DNF_set_cover}
The set cover instance $\mathcal{S}$ has a size-k set cover if and only if $\Gamma$ is a monotone conjunction of $k$ variables \violet{under $\mathcal{D}$}. 
\end{fact}

In particular, given any set cover $C\sse S$, the conjunction of the variables in $C$ corresponds to a monotone conjunction of $|C|$ variables that exactly computes $\Gamma$ over $\mathcal{D}$. Indeed, if $u\in U$, then $\mathcal{N}_\mathcal{S}(u)\cap C\neq\varnothing$ and so one of the $0$-coordinates of the encoded string $S\setminus \mathcal{N}_\mathcal{S}(u)$ intersects with the coordinates in $C$.

% \begin{fact}
% \label{fact:hittingset_disjunction}
% The set cover instance $\mathcal{S}$ has a size-$k$ set cover if and only if $\Gamma$ can be computed by a monotone disjunction of $k$ variables. 
% \end{fact}

% In particular, given any set cover $C\sse S$, the disjunction of the variables in $C$ corresponds to a monotone disjunction of $|C|$ variables that exactly computes $\Gamma$ over $\mathcal{D}$.


In order to obtain strong hardness results\lnote{``strong hardness results" is somewhat vague}, we use a parity amplification technique where we substitute parities into the evaluation of $\Gamma$. We first give a proof of hardness against learning this amplified function with decision tree targets\lnote{We mean hypotheses instead of targets here right? Same in next sentence.}. This proof illustrates the main conceptual ideas and will be leveraged in \Cref{section:lower_bounds_dt_estimation} to prove testing hardness. Then we generalize the proof to the setting of DNF targets. 

\begin{definition}[$\mathcal{D}_{\oplus \ell}$ and $\Gamma_{\oplus \ell}$]
%\label{def:Dl_and_Gammal}
Let $\mathcal{S}=(S,U,E)$ be a set cover instance with $|S|=n$. For $\ell\in\N$, the distribution $\mathcal{D}_{\oplus \ell}$ over strings in $\zo^{n\cdot\ell}$ is defined by sampling $\bx\sim \mathcal{D}$ and then for each $i\in[n]$ sampling $\by_i\sim \zo^{\ell}$ uniformly at random among all strings satisfying $\bigoplus \by_i=(\by_i)_1\oplus \cdots\oplus(\by_i)_\ell =\bx_i$. We then define $\Gamma_{\oplus \ell}:\supp(\mathcal{D}_{\oplus \ell})\to\zo$ by
$$
\Gamma_{\oplus \ell}(y_1,\ldots,y_n)=\Gamma\left(\oplus y_1,\ldots,\oplus y_n\right)
$$
where each $y_i\in\zo^\ell$. 
\end{definition}

\lnote{Let's move this up: we should introduce notation before using it.} In general, for $\by\sim \mathcal{D}_{\oplus \ell}$ we write $\by_i\in\zo^\ell$ for the $i$th ``block'' of $\by$ and $(\by_i)_j$ for the $j$th entry of the $i$th block. In general, for a string $y$, we write $\oplus y$ to denote the parity of the bits in $y$. For $y\in\zo^{n\cdot\ell}$, we write $\Oplus_n y$ to denote the string $(\oplus y_1,\ldots,\oplus y_n)\in\zo^n$.\cnote{Open to ideas for better notation.}\lnote{How about $\textnormal{BlockwisePar}(y)$?}

\lnote{Prose like this is good, but it is not clear to me what this sentence means.  Let's discuss.}The distribution $\mathcal{D}_{\oplus \ell}$ has the property that it parametrized by a bit index $j\in[\ell]$ and then factored into an ``outer'' uniform distribution and an ``inner'' distribution $\mathcal{D}$.

\begin{definition}[Alternative characterization of $\mathcal{D}_{\oplus\ell}$]
%\label{def:alternative_Dlj}
For $j\in[\ell]$, the distribution $\mathcal{D}_{\oplus\ell}^j$ is obtained via the following sampling procedure.
\begin{enumerate}
    \item Sample $(\by_1,\ldots,\by_n)\in\left(\zo^{(\ell-1)}\right)^n$ uniformly at random;
    \item sample $\bx\sim\mathcal{D}$;
    \item for each $i\in[n]$, fill in the $j$th bit of $\by_i$ so that $\bx_i=\oplus\by_i$.
\end{enumerate}
\end{definition}
For $y=(y_1,\ldots,y_n)\in\left(\zo^{(\ell-1)}\right)^n$ and $x\in\supp(\mathcal{D})$, we write $y^{\oplus(x,j)}\in\zo^{n\cdot\ell}$\cnote{Alternative notation ideas: $\Plus_j(y,x)\in\zo^{n\cdot\ell}$ or $y^{(j,x)}$ or $y^{+(x,j)}$ or $y^{+j\mid x}$.} for the string formed by filling in the $j$th bit of each $y_i$ so that $x_i=\oplus y_i$. 
\paragraph{Example.}\lnote{Examples are great.}{Consider $n=4$ and $\ell=3$ and $j=2$. Then, we can view $y=(y_1,\ldots,y_4)\in\supp(\mathcal{D}_{\oplus 3})$ as a $4\times 3$ matrix where the $i$th row is $y_i$. Likewise, we view $y=(y_1,\ldots,y_4)\in\left(\zo^{2}\right)^4$ as a $4\times 3$ matrix where the 2nd ($j=2$) column is ``undetermined'' (denoted below with $\star$) which is then ``filled in'' after selecting $x\in\zo^n$. In this case, we may have for example: 
$$
y=
\begin{bmatrix}
1 & \star & 0\\
0 & \star & 0\\
0 & \star & 1\\
1 & \star & 0
\end{bmatrix}\quad
x=
\begin{bmatrix}
1\\
1\\
0\\
1
\end{bmatrix}
\quad
\longrightarrow
\quad
y^{\oplus(x,j)}=
\begin{bmatrix}
1 & 0 & 0\\
0 & 1 & 0\\
0 & 1 & 1\\
1 & 0 & 0
\end{bmatrix}.
$$

}

\begin{proposition}[$\mathcal{D}_{\oplus\ell}^j$ is identical to $\mathcal{D}_{\oplus\ell}$]\lnote{Slightly strange to say that one distribution characterizes another -- not clear to me what that means. How about just saying that one distribution is identical (or equivalent) to the other, and in terms of notation, ``$\mathcal{D}_{\oplus \ell}^j \equiv \mathcal{D}_{\oplus \ell}$"?} 
For all $j\in[\ell]$ and $y\in\zo^{n\cdot\ell}$, 
$$
\pryd{\by=y}=\prydj{\by=y}
$$
\end{proposition}
\begin{proof}
Let $y=(y_1,\ldots,y_n)\in\left(\zo^\ell\right)^n$. Then we have
\begin{align*}
    \pryd{\by=y}&=\pryd{\Oplus_n\by = \Oplus_n y}\cdot\pryd{\by=y\mid \Oplus_n\by = \Oplus_n y}\tag{law of total probability}\\
    &=\prxd{\bx=\Oplus_n y}\cdot \underset{\by\sim \mathcal{U}_{n\cdot\ell}}{\Pr}\left[{\by=y\mid \Oplus_n\by = \Oplus_n y}\right]\tag{Definition of $\mathcal{D}_{\oplus \ell}$}\\
    &=\prxd{\bx=\Oplus_n y}\cdot \prod_{i\in[n]}\underset{\by_i\sim \mathcal{U}_{\ell}}{\Pr}\left[{\by_i=y_i\mid \oplus\by_i = \oplus y_i}\right]\tag{independence of $\by_i$}\\
    &=\prxd{\bx=\Oplus_n y}\cdot \prod_{i\in[n]}2^{-(\ell-1)}
\end{align*}
where the last step follows from the fact that conditioning on the parity of $\by_i$ being a specific bit removes $1$ degree of freedom from the uniformly random $\ell$ bits: $\by_i\sim\mathcal{U}_{\ell}$.\lnote{Minor, but I think writing $\by_i \sim \mathcal{U}_\ell$ here could be confusing. $\by_i$ is \emph{not} distributed uniformly in the proof right?}\cnote{Addressing the above comment: it is uniformly distributed under the conditional distribution. Conditioning is essential to prove the equivalence of the two distributions but after we've established the equivalence we no longer need to condition. I could add more to the prose if that'd help?} With an analogous calculation for $\mathcal{D}^j_{\oplus\ell}$, we obtain
\begin{align*}
    \prydj{\by=y}&=\prydj{\Oplus_n\by = \Oplus_n y}\cdot\prydj{\by=y\mid \Oplus_n\by = \Oplus_n y}\tag{law of total probability}\\
    &=\prxd{\bx=\Oplus_n y}\cdot\prod_{i\in[n]}\underset{\by_i\sim\mathcal{U}_{\ell-1}}{\Pr}\left[\by_i=y_i^{-j}\right]\tag{Definition of $\mathcal{D}_{\oplus \ell}^j$}\\
    &=\prxd{\bx=\Oplus_n y}\cdot \prod_{i\in[n]}2^{-(\ell-1)}
\end{align*}
where $y_i^{-j}\in\zo^{\ell-1}$ is the string $y_i$ with its $j$th bit removed.
\end{proof}
\lnote{Let's put everything above into a subsection titled ``The functions $\Gamma,\Gamma_{\oplus \ell}$, the distributions $\mathcal{D},\mathcal{D}_{\oplus \ell}$, and their basic properties."  At some point in this section we should discuss the circuit representation of $\Gamma_{\oplus \ell}$ (a depth-$3$ circuit with $\{ \oplus ,\vee\}$ gates regardless of set cover size) vs.~its true complexity under $\mathcal{D}$ (small junta if set cover is small).}  

\lnote{Start of new subsection here, maybe titled something like ``Warmup for~\Cref{lem:Set-Cover-to-DTs}: Decision tree hypotheses". Let's start the section by stating the analogue of~\Cref{lem:Set-Cover-to-DTs} that we'll prove.}

We are now able to prove that $\Gamma_{\oplus\ell}$ has a small decision tree if $\opt(\mathcal{S})$ is small and requires large decision trees even to approximate if $\opt(\mathcal{S})$ is large.
\begin{proposition}\lnote{Should we just state that it's a $\opt(\mathcal{S})\cdot \ell$ junta here?} 
\label{prop:gamma_small_depth}
Given an $N$-vertex set cover instance $\mathcal{S}=(S,U,E)$ with $|S|=n$ and parameter $\ell\in \N$, the function $\Gamma_{\oplus \ell}:\zo^{n\cdot\ell}\to\zo$ can be computed exactly by a decision tree of depth $\opt(\mathcal{S})\cdot \ell$. 
\end{proposition}

\begin{proof}
Let $C\sse S$ be a set cover with $|C|=\opt(\mathcal{S})$. Then $\Gamma_{\oplus\ell}$ is an $|C|\cdot \ell$-junta: $\Gamma_{\oplus\ell}(y)$ only depends on the blocks $y_i\in\zo^\ell$ for $i\in C$. Therefore, $\Gamma_{\oplus\ell}$ is exactly computed by the decision tree that exhaustively queries the $|C|\cdot\ell=\opt(\mathcal{S})\cdot\ell$ relevant variables. 
\end{proof}

\begin{theorem}[$\Gamma_{\oplus \ell}$ cannot be approximated by a small decision tree]
\label{thm:set_cover_reduction}
Given an $N$-vertex set cover instance $\mathcal{S}=(S,U,E)$ with $|S|=n$ and parameter $\ell\in \N$, for any decision tree $T$, if $|T|<2^{\opt(\mathcal{S}) {\ell}/8}$ then $\dist_{\mathcal{D}_{\oplus\ell}}(T,\Gamma_{\oplus\ell})\ge 1/(4N)$.
\end{theorem}

\subsubsection{Proof of~\Cref{thm:set_cover_reduction}}

We start by proving three properties about the functions $\Gamma,\Gamma_{\oplus\ell}$ and the corresponding distributions $\mathcal{D},\mathcal{D}_{\oplus\ell}$. The high level idea is to show the following.\lnote{Minor: let's reorder the claims in this section so that it matches the order here in this outline.}
\begin{enumerate}[itemsep=0.1em]
    \item No decision tree with small average depth can approximate $\Gamma$ \violet{under $\mathcal{D}$} (\Cref{claim:depth_error}).
    \item Any decision tree with small average depth that approximates $\Gamma_{\oplus \ell}$ \violet{under $\mathcal{D}_{\oplus \ell}$} can be used to construct \violet{decision tree of much smaller average depth} that approximates $\Gamma$ \violet{under $\mathcal{D}$}  (\Cref{claim:extracting_small_dt}).
    \item Any small size decision tree must have small average-depth (\Cref{claim:avg_depth}) \violet{with respect to $\mathcal{D}_{\oplus \ell}$}.
    \item Therefore, no small size decision tree can approximate $\Gamma_{\oplus\ell}$ \violet{under $\mathcal{D}_{\oplus \ell}$}.
\end{enumerate}
\gray{ Both ``approximate'' and ``average-depth'' are probabilistic quantities over the distributions $\mathcal{D}$ or $\mathcal{D}_{\oplus \ell}$.}

The first claim states that any small depth decision tree computing $\Gamma$ must have large error over the distribution $\mathcal{D}$.

\begin{claim}[Good approximators for $\Gamma$ require large depth]
\label{claim:depth_error}
Let $T$ be a decision tree on $n$ variables and $\mathcal{S}=(S,U,E)$ be an $N$-vertex set cover instance with $|S|=n$. If $\underset{\bx\sim D}{\E}[\depth_T(\bx)]<\opt(\mathcal{S})/2$ then $\dist_D(T,\Gamma)\ge 1/(2N)$.\lnote{$D \to \mathcal{D}$ througout.} 
\end{claim}

\begin{proof}
Let $T$ be a decision tree satisfying $\underset{\bx\sim D}{\E}[\depth_T(\bx)]<\opt(\mathcal{S})/2$. We actually prove the stronger claim that $\dist_{\mathcal{D}}(T,\Gamma)\ge 1/(2|U|)$. Suppose for contradiction that $\dist_{\mathcal{D}}(T,\Gamma)< 1/(2|U|)$. Each $x\in \supp(\mathcal{D})$ has mass $\ge 1/(2|U|)$ and so we must have $\dist_{\mathcal{D}}(T,\Gamma)=0$. Let $C\sse [n]=S$ be the set of vertices that $T$ queries in the computation of $1^n$ (equivalently, $C$ is the rightmost root-to-leaf path in $T$). We claim $C$ is a valid set cover for $\mathcal{S}$. Indeed, if some $u\in U$ is not covered by $C$, then $\mathcal{N}_\mathcal{S}(u)\cap C=\varnothing$ and so $u$ follows the same root-to-leaf path in $T$ as $1^n$. But such a $u$ yields a contradiction as $0=T(0^n)=T(u)$ and $1=\Gamma(1^n)\neq \Gamma(u)=0$ implies $\dist_\mathcal{D}(T,\Gamma)\ge 1/(2|U|)$. It follows that $C$ must be a valid set cover and $\opt(S)\le |C|$. 
We then have
\begin{align*}
    \underset{\bx\sim D}{\E}[\depth_T(\bx)]&\ge \underset{\bx\sim D}{\Pr}[x=1^n]\cdot |C|\tag{$\depth_T(1^n)=|C|$}\\
    &= \frac{|C|}{2}\\
    &\ge \frac{\opt(\mathcal{S})}{2}
\end{align*}
which contradicts our original assumption on the average-depth.
\end{proof}

In the next claim, we show that small decision trees must have small average depth over $\mathcal{D}_{\oplus\ell}$. To prove this claim, we need a lemma stating that the probability a string $\by\sim\mathcal{D}_{\oplus\ell}$ matches some fixed substring decays exponentially with the length of the substring.\lnote{Let's have a quick sentence contrasting with the bound one would get for truly uniform, to help give the reader some intuition.} 

\begin{lemma}[$\mathcal{D}_{\oplus\ell}$ is uniform-like]\cnote{later we will prove this claim for different distributions}
\label{lemma:avg_depth_lemma}
For all $R\sse [\ell]$ satisfying $|R|<\ell$ and for all $r\in\zo^{|R|}$, $i\in [n]$, and $x\in\supp(\mathcal{D})$, the distribution $\mathcal{D}_{\oplus \ell}$ on $\zo^{n\cdot\ell}$ satisfies
$$
\underset{\by\sim D_{\oplus\ell}}{\Pr}[(\by_i)_R=r\mid \Oplus_n\by=x]\le 2^{-|R|/2}
$$
where $(\by_i)_R\in\zo^{|R|}$ is the substring of $\by_i\in\zo^{\ell}$ consisting of the coordinates specified by $R$.
\end{lemma}

\begin{proof}
\red{ By the definition of $\mathcal{D}_{\oplus \ell}$, for any $b\in\zo$, the distribution of $\by_i$ conditioned on $\oplus \by_i=b$ is uniform over $\zo^\ell$. That is, we can write
$$
\underset{\by\sim \mathcal{D}_{\oplus\ell}}{\Pr}[(\by_i)_R=r\mid \oplus \by_i=b]=\frac{2^{\ell-|R|-1}}{2^{\ell-1}}=2^{-|R|}\le 2^{-|R|/2}
$$}
assuming $|R|<\ell$ since there are $2^{\ell-1}$ many strings in $\zo^\ell$ whose parity is $b$. 
If $|R|=\ell$, then 
$$\Pr[(\by_i)_R=r\mid \oplus \by_i=1-\oplus r]=0\qquad \Pr[(\by_i)_R=r\mid \oplus \by_i=\oplus r]=2^{-\ell+1}=2^{-|R|+1}.$$ 
In either case, we have the desired probability bound. The lemma then follows as the condition $\left[\Oplus_n\by=x\right]$ can equivalently be written as $[\oplus\by_i=x_i]$ due to the fact that given $x$, the $\by_i$ are sampled independently. 
\end{proof}

\begin{claim}[Small trees have small average depth]
\label{claim:avg_depth}
Let $T$ be a size-$s$ decision tree, then $$\underset{\by\sim \mathcal{D}_{\oplus \ell}}{\E}\left[\depth_T(\by)\right]\le 2\log(s).$$
\end{claim}

\begin{proof}
Let $L$ be a leaf in $T$ which we denote $L\in T$. The depth of $L$ in $T$ is $|L|$. Using this notation, we write the average depth as
\begin{equation}
\label{eq:avg_depth}
\underset{\by\sim \mathcal{D}_{\oplus \ell}}{\E}\left[\depth_T(\by)\right]=\sum_{L\in T}|L|\cdot \underset{\by\sim \mathcal{D}_{\oplus \ell}}{\Pr}[\by\text{ reaches }L].
\end{equation}
We start by upper bounding the quantity $\pryd{\by\text{ reaches } L}$. Write $L_i(y)$ for the substring of $y_i\in\zo^\ell$ queried along the root-to-leaf path to $L$ in $T$. Similarly, write $L_i$ for the set of variables $(y_i)_j$ for some $j\in[\ell]$ queried along the root-to-leaf path to $L$ in $T$. Thus, $L_i(y)$ is a substring of length $|L_i|$ and $\sum_{i\in[n]}|L_i|=|L|$. Once the string $x\in\zo^n$ is fixed, the strings $y_i$ are sampled independently at random. Therefore,
\begin{align*}
    \pryd{\by\text{ reaches } L\mid \oplus\by=x}&=\prod_{i\in[n]}\pryd{L_i(\by)=L_i\mid \Oplus_n\by=x}\\
    &\le \prod_{i\in[n]} 2^{-|L_i|/2}\tag{\Cref{lemma:avg_depth_lemma}}\\
    &= 2^{-|L|/2}.
\end{align*}

We can now compute
\begin{align*}
    \pryd{\by\text{ reaches } L}&=\sum_{x\in\supp(\mathcal{D})} \pryd{\Oplus_n\by = x}\cdot\pryd{\by\text{ reaches } L\mid \Oplus_n\by=x}\\
    &\le 2^{-|L|/2}\cdot \sum_{x\in\supp(\mathcal{D})} \pryd{\Oplus_n\by = x}\\
    &=2^{-|L|/2}.
\end{align*}

Referring back to \cref{eq:avg_depth}, we apply Jensen's inequality using the convex function $x\mapsto 2^{x/2}$ to the expected depth:
\begin{align*}
\red{    {\underset{\by\sim \mathcal{D}_{\oplus \ell}}{\E}\left[\depth_T(\by)\right]}\cdot \frac{1}2}&\red{\le \log\left(\eyd{2^{\depth_T(\by)/2}}\right)}\\
    &=\log\left(\sum_{L\in T}2^{|L|/2}\cdot \underset{\by\sim \mathcal{D}_{\oplus \ell}}{\Pr}[\by\text{ reaches }L]\right)\\
    &\le\log\left(\sum_{L\in T}2^{|L|/2}\cdot 2^{-|L|/2}\right)\\
    &=\log(s). \qedhere 
\end{align*}
\end{proof}
The next claim shows that a small-depth approximator for $\Gamma_{\oplus\ell}$ yields a much smaller-depth approximator for $\Gamma$. Our overall proof strategy is loosely inspired by \cite{BKLS20} which itself built on \cite{BB19}. This proof also crucially relies on \Cref{prop:Dj_equals_D} and the property that the distribution $\mathcal{D}_{\oplus\ell}$ is ``factorable''\lnote{Not clear to me what this means. Let's discuss}. 
\begin{claim}[Good approximators for $\Gamma_{\oplus\ell}$ yield good approximators for $\Gamma$]
\label{claim:extracting_small_dt}
Let $T$ be a decision tree such that $\dist_{\mathcal{D}_{\oplus \ell}}(T,\Gamma_{\oplus \ell})\le \eps$ and $\underset{\by\sim \mathcal{D}_{\oplus \ell}}{\E}[\depth_T(\by)]\le d$, then there is a restriction of the variables in $T$ which yields an $n$-variable decision tree $T'$ satisfying $\dist_\mathcal{D}(T',\Gamma)\le 2\eps$ and $\underset{\bx\sim \mathcal{D}}{\E}[\depth_{T'}(\bx)]\le 2d/\ell$.\lnote{Emphasize in prose before the claim that the approximator for $\Gamma$ has a much smaller depth. Let's also say that the overall strategy is inspired by Brody et al.'s proof, though the technical details differ.}
\end{claim}

\begin{proof}
Let $z=(z_1,\ldots,z_n)\in \left(\zo^{(\ell-1)}\right)^n$. Recalling the notation from \Cref{def:alternative_Dlj}, for $j\in[\ell]$, the string $z^{\oplus(j,x)}$ is formed by inserted a bit into the $j$th position of each $z_i$. Then, when $z$ and $j$ are fixed, the function $x\mapsto z^{\oplus(j,x)}$ is a well-defined function on $n$ bits. Our proof proceeds by finding a suitable $z\in\left(\zo^{(\ell-1)}\right)^n$ and $j\in[\ell]$ so that $x\mapsto T(z^{\oplus(j,x)})$ computes $\Gamma$ accurately over $\mathcal{D}$. Restricting $T$ according to the values specified by $z$ and $j$ yields the desired decision tree. 

For $j\in [\ell]$ and $y\in\zo^{n\cdot\ell}$, write $q_j(y)$ for the number of times that $T$ queries $(y_i)_j$ for some $i\in[n]$ on input the input $y$. Thus, $\depth_T(y)=\sum_{j\in[\ell]} q_j(y)$ and likewise
$$
\sum_{j\in[\ell]} \underset{\by\sim \mathcal{D}_{\oplus \ell}}{\E}[q_j(\by)]=\underset{\by\sim \mathcal{D}_{\oplus \ell}}{\E}[\depth_T(\by)]\le d.
$$
Let $\underline{j}\in [\ell]$ be the index that minimizes $\underset{\by\sim \mathcal{D}_{\oplus \ell}}{\E}[q_j(\by)]$. By averaging, this $\underline{j}$ must satisfy $\underset{\by\sim \mathcal{D}_{\oplus \ell}}{\E}[q_{\underline{j}}(\by)]\le d/\ell$. 

For any $j\in[\ell]$, we can write
\begin{align*}
    \eps&\ge\underset{\by\sim \mathcal{D}_{\oplus \ell}}{\E}[\Ind[T(\by)\neq \Gamma_{\oplus\ell}(\by)]]\\
    &=\underset{\by\sim \mathcal{D}^j_{\oplus \ell}}{\E}[\Ind[T(\by)\neq \Gamma_{\oplus\ell}(\by)]]\tag{\Cref{prop:Dj_equals_D}}\\
    &=\underset{\bz\sim \mathcal{U}_{n(\ell-1)}}{\E}\left[\underset{\bx\sim \mathcal{D}}{\E}\left[\Ind\left[T(\bz^{\oplus(\bx,j)})\neq \Gamma(\bx)\right]\right]\right].\tag{Definition of $\mathcal{D}_{\oplus\ell}^j$}
\end{align*}
In particular, for $\underline{j}$ we have 
\begin{align*}
    \underset{\bz\sim \mathcal{U}_{n(\ell-1)}}{\E}\left[\underset{\bx\sim \mathcal{D}}{\E}\left[\Ind \left[T(\bz^{\oplus(\bx,\underline{j})})\neq \Gamma(\bx)\right]\right]\right]&\le\eps\\
    \underset{\bz\sim \mathcal{U}_{n(\ell-1)}}{\E}\left[\underset{\bx\sim \mathcal{D}}{\E}\left[q_{\underline{j}}(\bz^{\oplus(\bx,\underline{j})})\right]\right]&\le\frac{d}{\ell}
\end{align*}
By Markov's inequality,
\begin{align*}
    \underset{\bz\sim \mathcal{U}_{n(\ell-1)}}{\Pr}\left[\underset{\bx\sim \mathcal{D}}{\E}\left[\Ind\left[T(\bz^{\oplus(\bx,\underline{j})})\neq \Gamma(\bx)\right]\right]>2\eps\right]&<\frac{1}{2}\\
    \underset{\bz\sim \mathcal{U}_{n(\ell-1)}}{\Pr}\left[\underset{\bx\sim \mathcal{D}}{\E}\left[q_{\underline{j}}(\bz^{\oplus(\bx,\underline{j})})\right]>2d/\ell\right]&<\frac{1}{2}.
\end{align*}
And thus by a union bound, there is some fixed $\underline{z}\in \zo^{n(\ell-1)}$ satisfying
\begin{align*}
    \underset{\bx\sim \mathcal{D}}{\E}\left[\Ind[T({\underline{z}}^{\oplus(\bx,\underline{j})})\neq \Gamma(\bx)]\right]&\le 2\eps\\
    \underset{\bx\sim \mathcal{D}}{\E}\left[q_{\underline{j}}({\underline{z}}^{\oplus(\bx,\underline{j})})\right]&\le 2d/\ell.
\end{align*}
The tree $T'$ can be formed by restricting $T$ according to the string $\underline{z}$. Also, this tree $T'$ satisfies $\depth_{T'}(x)=q_{\underline{j}}({\underline{z}}^{(\bx,\underline{j})})$ by construction. The claim then follows.
\end{proof}


\paragraph{Putting things together: Proof of~\Cref{thm:set_cover_reduction}}. Suppose there is some tree $T$ computing $\Gamma_{\oplus \ell}$ with $|T|\le 2^{\opt(\mathcal{S})\ell/8}$. We show that $\dist(T,\Gamma_{\oplus \ell})\ge 1/(4N)$. Suppose for contradiction that $\dist(T,\Gamma_{\oplus\ell})<1/(4N)$. By \Cref{claim:avg_depth}, we have $\eyd{\depth_T(\by)}< 2\cdot\log\left(2^{\opt(\mathcal{S})\ell/8}\right)=\opt(\mathcal{S})\ell/4$. Then by \Cref{claim:extracting_small_dt} there is a decision tree $\hat T$ satisfying
$$
\dist_\mathcal{D}(\hat T,\Gamma)< \frac{1}{2N}\qquad \underset{\bx\sim \mathcal{D}}{\E}[\depth_{\hat T}(\bx)]< \frac{\opt(\mathcal{S})}{2}.
$$
But this contradicts \Cref{claim:depth_error}.
}
